Spherical function regularization for parallel MRI reconstruction

From the optimization point of view, a difficulty with parallel MRI with simultaneous coil sensitivity estimation is the multiplicative nature of the non-linear forward operator: the image being reconstructed and the coil sensitivities compete against each other, causing the optimization process to be very sensitive to small perturbations. This can, to some extent, be avoided by regularizing the unknown in a suitably "orthogonal" fashion. In this paper, we introduce such a regularization based on spherical function bases. To perform this regularization, we represent efficient recurrence formulas for spherical Bessel functions and associated Legendre functions. Numerically, we study the solution of the model with non-linear ADMM. We perform various numerical simulations to demonstrate the efficacy of the proposed model in parallel MRI reconstruction.

==> texbase/highlightname.tex <==
%\addbibresource{\jobname.bib}
\newcommand*{\mknamesignature}[5]{\edef#1{(#2|#3|#4|#5)}}
\mknamesignature{\highlightname}{DISABLEDValkonen}{DISABLEDTuomo}{}{}
\def\highlightfamily{Valkonen}
\def\ancientversion{2.8a}
% mbox needed to not make next character automatically  upper case
\providecommand{\shortform}{\mbox{T.\,V.}}
\makeatletter

\ifdefequal{\abx@version}{\ancientversion}{
	\DeclareNameFormat{labelname}{%
	  \begingroup
	  \mknamesignature{\currentsignature}{#1}{#3}{#5}{#7}%
	  \ifdefequal{\highlightname}{\currentsignature}%
	    {\let\mkbibnamefirst=\@gobble%
	     \def\mkbibnamelast{\shortform\@gobble}%
	     \let\mkbibnameprefix=\@gobble%
	     \let\mkbibnameaffix=\@gobble}%
	    {\let\mkbibnamefirst=\@gobble}%
	  \ifcase\value{uniquename}%
	    \usebibmacro{name:last}{#1}{#3}{#5}{#7}%
	  \or
	    \ifuseprefix
	      {\usebibmacro{name:first-last}{#1}{#4}{#5}{#8}}
	      {\usebibmacro{name:first-last}{#1}{#4}{#6}{#8}}%
	  \or
	    \usebibmacro{name:first-last}{#1}{#3}{#5}{#7}%
	  \fi
	  \endgroup
	  \usebibmacro{name:andothers}%
	}
}{
	\DeclareNameFormat{labelname}{%
	  \nameparts{#1}%
	  \begingroup%
	  \mknamesignature{\currentnamex}{\namepartfamily}{\namepartgiven}{\namepartprefix}{\namepartsuffix}%
	  \ifdefstrequal{\highlightname}{\currentnamex}%
	    {%
	      \usebibmacro{name:delim}{\shortform}%
	      \shortform%
	    }{%
	      \usebibmacro{name:family}
	           {\namepartfamily}
	           {\namepartgiven}
	           {\namepartprefix}
	           {\namepartsuffix}%
	    }%
	  \endgroup%
	  \usebibmacro{name:andothers}
	}
}
\makeatother

\DeclareNameAlias{default}{labelname}


==> texbase/symbols-common.tex <==


\let\polishL=\L

\newcommand{\term}{\emph}

\newcommand{\field}[1]{\mathbb{#1}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\field{Q}}
\newcommand{\R}{\field{R}}
\newcommand{\extR}{\overline \R}
%\newcommand{\B}{\mathbb{B}}
\newcommand{\B}{B}
\newcommand{\Bclosed}{{\overline B}}
\newcommand{\Sphere}{S}
\newcommand{\Rinf}{\overline{\field{R}}}
\newcommand{\Rplusinf}{\field{R}_{+\infty}}
\newcommand{\Complex}{\field{C}}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\adaptnorm}[1]{\left\|#1\right\|}
\newcommand{\bignorm}[1]{\bigl\|#1\bigr\|}
\newcommand{\Bignorm}[1]{\Bigl\|#1\Bigr\|}
\newcommand{\abs}[1]{|#1|}
\newcommand{\adaptabs}[1]{\left|#1\right|}
\newcommand{\bigabs}[1]{\bigl|#1\bigr|}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\grad}{\nabla}
\newcommand{\freevar}{\,\boldsymbol\cdot\,}
\newcommand{\cconj}[1]{\overline{#1}}
%\renewcommand{\vec}[1]{\boldsymbol #1}
\newcommand{\Union}\bigcup
\newcommand{\Isect}\bigcap
\newcommand{\union}\cup
\newcommand{\isect}\cap
\newcommand{\bigunion}\bigcup
\newcommand{\bigisect}\bigcap
\newcommand{\powerset}{\mathcal{P}}
\newcommand{\defeq}{:=}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\downto}{\searrow}
\newcommand{\upto}{\nearrow}
\newcommand{\subdiff}{\partial}
\newcommand{\rangeSymbol}{\mathcal{R}}
\newcommand{\range}[1]{\rangeSymbol(#1)}
\newcommand{\rsg}[1]{\mathcal{R}(\subdiff #1)}
\newcommand{\pinv}[1]{#1^\dag}

%\newcommand{\forallx}{\text{ for all }}

%\newcommand{\BB}{\mathbb{B}}
%\newcommand{\FF}{\mathcal{F}}

\newcommand{\MIN}[1]{{\underline {#1}}}
\newcommand{\MAX}[1]{{\overline {#1}}}

\DeclareMathOperator*{\lip}{lip}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\epsargmin}{\epsilon-arg\,min}
\newcommand{\epsargmin}[1][\epsilon]{\operatorname{#1-arg\,min}}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\ri}{ri}
\DeclareMathOperator{\rbd}{rbd}
\DeclareMathOperator{\closure}{cl}
\DeclareMathOperator{\bd}{bd}
\DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Dom}{dom}
\DeclareMathOperator{\Cod}{cod}
\DeclareMathOperator{\lev}{lev}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\epi}{epi}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\graph}{Graph}
\DeclareMathOperator{\cond}{cond}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\esssup}{ess\,sup}
\DeclareMathOperator{\support}{supp}
\DeclareMathOperator{\divergence}{div}

\makeatletter
\def \uminus@sym{\setbox0=\hbox{$\cup$}\rlap{\hbox 
        to\wd0{\hss\raise0.5ex\hbox{$\scriptscriptstyle{-}$}\hss}}\box0}
    \def \uminus    {\mathrel{\uminus@sym}}
\makeatother

\newcommand{\mathvar}[1]{\textup{#1}}

\newcommand{\iprod}[2]{\langle #1,#2\rangle}
\newcommand{\adaptiprod}[2]{\left\langle #1,#2\right\rangle}

\newcommand{\weakto}{\mathrel{\rightharpoonup}}
\makeatletter
\def \weaktostar@sym{\setbox0=\hbox{$\rightharpoonup$}\rlap{\hbox 
        to\wd0{\hss\raise1ex\hbox{$\scriptscriptstyle{*\,}$}\hss}}\box0}
    \def \weaktostar    {\mathrel{\weaktostar@sym}}
\makeatother


==> texbase/symbols-ip.tex <==

%\usepackage{undertilde}

\newcommand{\jprod}{\circ}
\newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\iK}{\interior \K}
\newcommand{\E}{\mathcal{E}}
\newcommand{\Neigh}{\mathcal{C}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\nullspace}[1]{\mathcal{N}(#1)}
%\newcommand{\iprod}[2]{\langle #1,#2\rangle}
\newcommand{\Pep}{P_e^\perp}
\newcommand{\DC}{\mathrm{DC}}
\newcommand{\extsubdiff}{\widehat \subdiff}
\newcommand{\subdiffDC}{\subdiff^\DC}
\newcommand{\extsubdiffDC}{\extsubdiff^\DC}
\newcommand{\polar}[1]{{#1}^\circ}
\newcommand{\bipolar}[1]{{#1}^{\circ\circ}}
\newcommand{\regnormal}{\widehat N}
\newcommand{\regtangent}{\widehat T}
\newcommand{\HG}{{\widehat G}}
\newcommand{\HU}{{\widehat U}}
\newcommand{\IG}{\inv G}
\newcommand{\IHG}{\inv \HG}
%\newcommand{\varsym}{\bullet}
\newcommand{\wtilde}{\widetilde}
%\newcommand{\setto}{\rightrightarrows}

%\renewcommand{\norm}[1]{\|#1\|}
%\newcommand{\adjnorm}[1]{\left\|#1\right\|}

\newcommand{\eigval}{\lambda}
%\newcommand{\eigvaltwo}{\zeta}

\newcommand{\Arw}{\mathrm{Arw}}


==> texbase/symbols-mna.tex <==

\newcommand{\mna}{\phi}
\newcommand{\plusmna}{\oplus}
\newcommand{\minusmna}{\ominus}
\newcommand{\iprodmna}{\odot}
%\DeclareMathOperator{\plusmna}{\hat +}
%\DeclareMathOperator{\minusmna}{\hat{--}}
%\DeclareMathOperator{\iprodmna}{\hat \times}
\newcommand{\Rmna}{\R_\mna}
\newcommand{\maybeeq}{\stackrel{?}{=}}
\newcommand\rhodom\sqsubset
\newcommand\rhodominv\sqsupset
\newcommand\rhodomneq{\sqsubset_{!}}
\newcommand\rholub\sqcup
\newcommand\rhoglb\sqcap
\newcommand{\sumop}{\biguplus}
\newcommand{\sumz}{\biguplus}
\newcommand{\plusz}{\uplus}
\newcommand{\minusz}{\uminus}
\newcommand{\pz}{\zeta}


==> texbase/symbols-ten.tex <==

\renewcommand{\tilde}{\widetilde}
\renewcommand{\ae}{a.e.~}
\DeclareMathOperator{\Sym}{Sym}
\newcommand{\Tensor}{\mathcal{T}}
\newcommand{\BDspace}{\mathvar{BD}}
\newcommand{\SBDspace}{\mathvar{SBD}}
\newcommand{\BVspace}{\mathvar{BV}}
\newcommand{\SBVspace}{\mathvar{SBV}}
\newcommand{\Eabs}{\mathcal{E}}
\newcommand{\Ejump}{E^j}
\newcommand{\Ecantor}{E^c}
\newcommand{\Meas}{\mathcal{M}}
\newcommand{\Distrib}{\mathcal{D}'}
\renewcommand{\H}{\mathcal{H}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\restrict}{\llcorner}
\newcommand{\BD}{\partial}
\renewcommand{\d}{\,d} %\text{d}}
\newcommand{\SymOp}{|\hspace{-1.5pt}|\hspace{-1.5pt}|}
\newcommand{\TGV}{\mathvar{TGV}}
\newcommand{\TV}{\mathvar{TV}}
\newcommand{\TD}{\mathvar{TD}}
\newcommand{\nonsym}{\text{ns}}
\newcommand{\sym}{\text{s}}
%\newcommand{\TVnonsym}{\TV^{\nonsym}}
%\newcommand{\TVsym}{\TV^{\sym}}
\newcommand{\TVsym}{\TD}
\newcommand{\TVnonsym}{\TV}
\newcommand{\TVlog}{\mathvar{logTV}}%{TV^{\log}}
\newcommand{\FA}{\text{FA}}
\newcommand{\BALL}{V}



==> texbase/texbase.tex <==
%\usepackage{footmisc}
\usepackage{bbm}
%\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mdframed}

\makeatletter
\newenvironment{taggedsubequations}[1]
 {%
  % \end{subequations} will advance `equation`
  \addtocounter{equation}{-1}%
  \begin{subequations}%
  % set the current label
  \def\@currentlabel{#1}%
  % redefine \theequation
  \renewcommand{\theequation}{#1.\alph{equation}}%
 }
 {\end{subequations}}
\makeatother %not \makeatletter

% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{conjecture}{Conjecture}

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
% \newtheorem*{assumption*}{Assumption}
% \newtheorem{remark}{Remark}
% \newtheorem*{remark*}{Remark}
% \newtheorem*{definition*}{Definition}
% \newtheorem{example}{Example}
% \newtheorem{algorithm}{Algorithm}

% \numberwithin{equation}{section}
% \numberwithin{lemma}{section}
% \numberwithin{theorem}{section}
% \numberwithin{proposition}{section}
% \numberwithin{definition}{section}
% \numberwithin{remark}{section}
% \numberwithin{example}{section}
% \numberwithin{assumption}{section}
% \numberwithin{algorithm}{section}
% \numberwithin{corollary}{section}

\mdfdefinestyle{examplebg}{
    backgroundcolor=black!7,%
    hidealllines=true,%
    innertopmargin=-.3em,%
    innerbottommargin=.7em,%
    innerleftmargin=.7em,%
    innerrightmargin=.7em,%
}

\surroundwithmdframed[style=examplebg]{example}
\surroundwithmdframed[style=examplebg]{algorithm}

% \makeatletter
% \AtBeginDocument{
%     \hypersetup{
%         pdftitle = {\@title},
%         pdfauthor = {\@author}
%     }
% }
% \makeatother

%\def\email#1{\texttt{\href{mailto:#1}{#1}}}

%%% define a new counter and use it for \theHequation which hyperref uses for the links
\newcounter{Hequation}
\renewcommand{\theHequation}{HREF.EQ.\arabic{Hequation}}
\makeatletter
\g@addto@macro\equation{\stepcounter{Hequation}}
\makeatother

% \makeatletter
%   \def\make@df@tag@@#1{%
%     \gdef\df@tag{%
%       \maketag@@@{\Hy@make@anchor#1}%
%       \def\@currentlabel{#1}%
%       \def\cref@currentlabel{[equation][2147483647][]#1}%
%     }%
%   }
%   \def\make@df@tag@@@#1{%
%     \gdef\df@tag{%
%       \tagform@{\Hy@make@anchor#1}%
%       \toks@\@xp{\p@equation{#1}}%
%       \edef\@currentlabel{\the\toks@}%
%       \edef\cref@currentlabel{[equation][2147483647][]\the\toks@}
%     }%
%   }
% \makeatother



==> texbase/todo.tex <==
% \usepackage{soul}

% \newcommand{\TODO}[1]{{\sethlcolor{magenta}\color{white}\bfseries\em\hl{#1}}}
\newcommand{\TODOX}[1]{{%
\colorbox{magenta}{\color{white}\bfseries\em#1}
}}

\usepackage[textsize=footnotesize,color=DarkOrange!40]{todonotes}
%\newcommand{\tvtodo}[2][]{\tikzexternaldisable\todo[color=DarkBlue!40,#1]{#2}\tikzexternalenable}
\newcommand{\TODO}[1]{\todo[inline]{#1}}


